Scientific Language Models for Biomedical Knowledge Base Completion: An Empirical Study

Biomedical knowledge graphs (KGs) hold rich information on entities such as diseases, drugs, and genes. Predicting missing links in these graphs can boost many important applications, such as drug design and repurposing. Recent work has shown that general-domain language models (LMs) can serve as "soft" KGs, and that they can be fine-tuned for the task of KG completion. In this work, we study scientific LMs for KG completion, exploring whether we can tap into their latent knowledge to enhance biomedical link prediction. We evaluate several domain-specific LMs, fine-tuning them on datasets centered on drugs and diseases that we represent as KGs and enrich with textual entity descriptions. We integrate the LM-based models with KG embedding models, using a router method that learns to assign each input example to either type of model and provides a substantial boost in performance. Finally, we demonstrate the advantage of LM models in the inductive setting with novel scientific entities. Our datasets and code are made publicly available.

==> 02_related.tex <==

\section{Related Work}
% \paragraph{KG embedding.} A dominant class of methods used for KG completion is KG embedding (KGE) models, which learn a dense vector representation of every entity and relation in the KG and combine these vectors to score the plausibility of each potential fact, represented as a triple of a head entity, relation, and tail entity (see Section \ref{subsec:methods}).
% These include methods that model a relation as a translation in a high-dimensional vector space, such as TransE \citep{bordes2013transe} and its variants \citep{wang2014transh, lin2015transr}, or a rotation in a complex vector space, such as the more modern method RotatE \citep{sun2019rotate} that addresses the inability of TransE to capture certain classes of relations. A plausibility score can also be generated via products of entity and relation vectors, with methods such as DistMult \citep{yang2015distmult} and ComplEx \citep{trouillon2016complex}.
% KGE methods have been widely explored in the general domain through evaluation on benchmark datasets derived from sources such as WordNet \citep{miller1995wordnet} and Freebase \citep{bollacker2008freebase}, and their utility has also recently been explored in the biomedical domain \citep{chang2020benchmark, alshahrani2021application, bonner2021understanding}.


% \paragraph{Text-based KG completion.} %A key shortcoming of KGE models is that they ignore additional metadata such as text associated with entities and relations.
% Some KG completion approaches use embeddings of textual descriptions of entities or relations, often to augment a KGE-based approach through joint loss functions that encourage the structure- and text-based representations to lie in the same embedding space \citep{wang2014jointly, toutanova2015representing, han2016jointrep, wang2016teke, xu2017kgrjointly}. Recent approaches such as KG-BERT \citep{yao2019kg} and variants \citep{kim2020mtkgbert,wang2021structure,daza2021blp} fine-tune the BERT language model (LM) \citep{devlin2019bert} for the task of KG completion using different loss functions and text encodings. Unlike previous work, %which evaluates on the same general domain benchmarks,
% we explore KG completion for \textit{biomedical} KGs using \textit{domain-specific} scientific LMs \citep{lee2020biobert, alsentzer2019bioclinicalbert, beltagy2019scibert, gu2020pubmedbert}. 
% Existing approaches in the general domain ensemble KGE and LM-based models, using a weighted average of their outputs \citep{wang2021structure}. We perform a thorough investigation of KGE and LM-based models, finding that an approach which adaptively selects a \textit{single} model to evaluate each example performs better than a weighted average, and that integrating two LMs can further boost results. %Given the ability of text-based approaches to attempt to perform KG completion with entities unseen during training
% Previous work has explored the potential for applying text-based approaches in the inductive setting with entities unseen during training \citep{xie2016dkrl, daza2021blp}. We study this setting in the biomedical domain, and also present a simple technique that allows KGE models to be used in the inductive setting by imputing missing entities with textually similar entities.  %We demonstrate the usefulness of LMs for inductive KG completion in the biomedical domain as well, and also explore using language to allow standard KGE models to be used in the inductive setting with a simple imputation technique based on textual entity representations.

% \paragraph{Biomedical LM.} There are a number of existing LMs that augment BERT with additional pretraining on various biomedical corpora, demonstrating that this improves performance on diverse natural language understanding (NLU) tasks \citep{lee2020biobert, alsentzer2019bioclinicalbert, beltagy2019scibert, gu2020pubmedbert}. However, the application of these domain-specific LMs has largely been limited to NLU tasks, and their utility for biomedical KG completion has been underexplored, with one recent work \citep{zhang2021drugrep} applying one LM model to relations extracted from COVID-19 papers.

% One notable exception applies StAR with a BioBERT base to drug repurposing for COVID-19 \citep{zhang2021drugrep}, but they perform no additional tuning of the model and report much worse performance compared to KGE-based methods. In contrast, we apply a wide range of biomedical LMs to multiple datasets, demonstrating comparable performance to KGE methods with proper hyperparameter tuning with additional benefits from integrating KGE and LM-based methods.


% \paragraph{} Existing text-for-KG-completion approaches have recognized the benefit of ensembling KGE models and text-based models, typically by using a weighted average of their outputs \citep{xie2016dkrl, wang2021structure}. We extend this work by performing a more thorough investigation of different methods for integrating KGE and LM-based models, and find that an approach which adaptively selects a single model to evaluate each example performs better than a weighted average approach. 



% \begin{itemize}
%     \item General domain knowledge graph completion methods, including: knowledge graph embeddings (e.g., TransE, ComplEx); shallow neural networks (e.g., NTN, ConvE); and pretrained language models (e.g., KG-BERT, StAR, BLP)
%     \item Older methods for KG completion that use text but don't use pretrained LMs (e.g., Kristina Toutanova's work, DKRL, ConMask)
%     \item Pretrained language models for biomedical NLP: BioBERT, Bio+ClinicalBERT, SciBERT, PubMedBERT
%     \item Existing work on biomedical KG completion with KGE models (drug repurposing for COVID-19 paper that uses StAR/STELP, recent William Hamilton papers on arXiv, etc.)
% \end{itemize}




==> ensemble.tex <==
\section{Ensembling}

\subsection{Ensembling results}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/router-repodb.png}
    \includegraphics[width=\textwidth]{fig/router-hetionet.png}
    \includegraphics[width=\textwidth]{fig/router-msi.png}
    \caption{\tom{do we need all four?}}
    \label{fig:ensemble}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/feature-importance-top10-repodb.png}
    \caption{rotate x axis tick lables; punctuation --> punct.; characters --> chars.; distance -> dist;}
    \label{fig:featimp}
\end{figure}

The ensembling results are summarized in Fig.~\ref{fig:ensemble}. We report only the results for the router method of ensembling, as this generally performs better than the input-dependent weighted average; the full set of ensembling results can be viewed in the Appendix. We observe that ensembling consistently improves test set MRR across all pairs of methods, although the magnitude of improvement varies depending on the choice of classifier, ensembling strategy, and pair of base models used. The best-performing ensemble in all cases involves PubMedBERT and a KGE model, demonstrating the benefit of augmenting a model that uses KG structure alone with one that makes use of entity text information. In contrast to previous work which only explores ensembling a text-based model with a KGE model, we demonstrate here that the largest improvement is not just a result of combining any pair of KG completion models but that including a text-based model uniquely contributes to maximizing gains in performance. We see in general that using a feature-based approach outperforms a simple feature-agnostic global average, and that the best-performing ensemble for each dataset uses a router as opposed to an input-dependent weighted average of ranking scores. 

To examine which features are most predictive of whether an LM or KGE model will perform well on a particular triple, we plot the top-10 XGBoost feature importances for all datasets in Fig.~\ref{fig:featimp}. 

\tom{analysis showing feature importance -- if we figure out those error bars --, what kind of examples get routed to kge vs. lm, or to one lm vs. another lm... etc.}

\tom{show examples (cherry picked) demonstrating some of the main feature-importance obersvations... e.g., some nodes with high page rank or in/out degree}

\rahul{potentially also include results ensembling multiple LMs (have to decide what to include - all pairs of LMs? Best and second best? Also include best KGE model (i.e., three-model ensemble)?)}\tom{yes! i'd include only the best and second best three-model combo per dataset, and maybe also the best + second best two-lm combo. and give some info in the text/appendix about the rest.}

\tom{consider adding regression analysis -- predicting the delta in rr (or something along those lines), to potentially get more clear cut results}

% \begin{itemize}
%     \item Ensembling best LM with best baselines improves results, with varying improvement across datasets
%     \item Best ensemble is almost always combination of a KGE model and an LM, rather than two KGE models
%     \item (Possibly) Also include results ensembling multiple LMs, or multiple LMs and a KGE model? \tom{if this helps results, then sure! we haven't seen others doing this}
% \end{itemize}

==> outline.tex <==
\begin{itemize}
    \item Knowledge graph completion is a well-studied problem, typically addressed with methods that only make use of the graph structure
    \item The huge success of pretrained language models on a wide variety of NLP tasks has led to them being adapted for KG completion (e.g., KG-BERT, StAR, BLP)
    \item In parallel, we have seen the development of domain-specific pretrained language models, including several for the biomedical domain (e.g., BioBERT, SciBERT, PubMedBERT)
    \item The biomedical domain is important for KG completion as well (e.g., drug repurposing, generating protein-protein interaction candidates for laboratory experiments) 
    \item However, most existing approaches for biomedical KG completion rely on the aforementioned graph structure-based KG completion methods, without making use of language \tom{maybe tone this one down a bit, even though you do say 'most' -- we know of word embedding methods that have been used; also, UMLS is strictly speaking a type of biomedical KG -- can anticipate this question and briefly say why it's not/different/limited/etc.} and without leveraging modern domain-specific pretrained LMs \tom{does domain-specific refer to 'biomedicine' broadly? or do we have evidence about different biomed/scientific LMs being better per dataset? or is pubmedbert always better?}
    \item We explore the use of biomedical LMs for KG completion, augmenting three existing datasets with entity names/descriptions and structuring them for KG completion training/evaluation, \tom{we find that as in previous work, the use of LMs falls short of graph-based models} and explore ensembles of classical KG embedding methods with newer biomedical LMs to improve KG completion performance \tom{re ensembling, do we have any interesting result/finding/insight that can differentiate us from previous work showing ensembles are needed? how about the router? multiple lms? characterizing cases where lm/kge each do better? can we show in which cases the ensemble is particularly helpful?}
    \item (Could also mention something about how domain-specific pretrained LMs might store information about biomedical entities in their parameters that could help with KG completion, but not sure if our current experiments confirm that this is happening) \tom{this or experiments with similar flavor could be a big boost}
    
    \item \tom{any interesting ablation experiments we can discuss?}
    
    \item \tom{error analysis? showing where there is potential for future research in this area.}
    
    
\end{itemize}

\section{Related Work}

\begin{itemize}
    \item General domain knowledge graph completion methods, including: knowledge graph embeddings (e.g., TransE, ComplEx); shallow neural networks (e.g., NTN, ConvE); and pretrained language models (e.g., KG-BERT, StAR, BLP)
    \item Older methods for KG completion that use text but don't use pretrained LMs (e.g., Kristina Toutanova's work, DKRL, ConMask; is it necessary to include this in the related work?)
    \item Pretrained language models for biomedical NLP: BioBERT, Bio+ClinicalBERT, SciBERT, PubMedBERT
\end{itemize}

\section{Datasets}

\begin{itemize}
    \item Three datasets, covering a range of different sizes (within the range of existing general domain KG completion benchmarks), various entity/relation types, and diverse biomedical knowledge base sources \tom{aside from their sizes, would be good to find interesting structural differences between these datasets -- in terms of entity names (avg length?), and basic graph properties. a table would be good. }
    \item Most of these datasets have not previously been used for knowledge graph completion, and none of them for KG completion using language (most don't even provide entity names *and* descriptions)
    \item We scraped entity names/descriptions and use them for training text-based KG completion methods (we plan to release the datasets, all entity names/descriptions, and our train/test splits to promote reproducibility)
    \item Include table with dataset statistics (size of training, validation, and test sets, number of entities and relations, sources)
    \item RepoDB: used for drug repurposing, contains drug-disease pairs approved for clinical use
    \item Hetionet: heterogeneous biomedical knowledge graph, previously used for KG completion but not with natural language; we use a subset that contains "drug treats disease", "disease presents with symptom", "disease is associated with gene", and "compound causes side effect" relations
    \item MSI (multiscale interactome): used for drug repurposing by exploring paths connecting different biomedical entities, published in Nature paper in March; contains drug-protein, disease-protein, protein-protein, protein-function, function-function, and drug-disease relations
\end{itemize}

\subsection{Knowledge Graph Completion}

\subsubsection{Task}

\begin{itemize}
    \item Overview of task: train a model that assigns a score to each $(h, r, t)$ triple, use scores to rank each positive test triple against a large set of negatives, compute ranking metrics
    \item Use negative samples for contrastive loss function, construct negatives by randomly corrupting head/tail entity with another entity of the same type
\end{itemize}

\subsubsection{Models}
\tom{add description of how you encode the triples (including SEP/CLS notations)}
\begin{itemize}
    \item Four knowledge graph embedding-based baselines spanning range of different score functions, all are still commonly used and several maintain competitive performance on general domain benchmarks: TransE, DistMult, ComplEx, RotatE
    \item Four (five?) biomedical pretrained language models, trained like KG-BERT: BioBERT, Bio+ClinicalBERT, SciBERT, PubMedBERT(, RoBERTa)
    \item Multi-task training seems to improve KG-BERT performance based on existing literature, so using multi-task loss for BERT models (include ablation analysis? Or not necessary since multi-task KG-BERT paper already does this?)
    \item For baselines, use max-margin ranking loss and perform hyperparameter search over: embedding dimension, margin, learning rate, number of negative samples, regularization
    \item For LMs, use multi-task loss and perform hyperparameter search over: batch size, learning rate.
    \item LMs use biomedical pretrained LM (e.g., PubMedBERT) as base model, use CLS token as representation of triple which is passed through three different linear layers for each of the three different tasks (loss function in parentheses): binary classification for link prediction (binary cross entropy); multiclass classification for relation prediction (cross entropy); and outputting a score for relevance ranking (max-margin)
\end{itemize}

\section{Experimental Results}
\tom{what parallels do we see with results in general domain? what differences in results? missing descriptions is one example difference -- btw did you make sure WN/FB don't have missing descriptions? -- would be nice to have more differences.}
\subsection{Individual models}
\tom{error analysis as motivating the ensemble would be good -- showing lm and kge have different correct predictions (if they have overlapping \textit{errors}, even better )}

\tom{we have seen some distinct properties differentiating the examples lm vs. kge each do better on -- need to report this and discuss}
\begin{itemize}
    \item Performance of language models is sometimes competitive with baselines and even better than some, but generally not better than best baseline (gap in performance differs across datasets)
    \item Maybe include some examples for one dataset where LMs/baselines do well/poorly?
    \item (Possibly) Unlike general domain, descriptions do not exist for all entities in these datasets (show performance on examples with/without descriptions for each class of method)
    \item Language models and knowledge graph embeddings seem to perform well on disjoint sets of examples (show bar plot with percentages of examples where each model performs best); motivates ensembling
\end{itemize}

\subsection{Ensembling}

\subsubsection{Methods}

\begin{itemize}
    \item Explore multiple different methods of ensembling a knowledge graph embedding model with a language model to boost overall performance
    \item Simplest method: global weighted average of LM and KGE ranking scores, weights chosen to maximize validation set MRR
    \item Classifier method: train a classifier on the validation set to predict whether the KGE model or the LM will perform better on a particular example, using ranking scores as well as features of the positive example (text-based, graph-based; list features here or in Appendix?) \tom{list some here -- or some higher-level categorization of the features --, since they are semi-interesting and we haven't seen others do this}
    \item Classifier can be trained as a router (send each example to one model or the other for ranking), or can use the output probabilities as input-dependent weights for weighted average of ranking scores
    \item Explore multiple classifiers of varying levels of complexity (logistic regression, XGBoost, MLP)
    \item Perform hyperparameter search for each of the classifiers (details in Appendix)
\end{itemize}

\subsubsection{Ensembling results}
\tom{analysis showing feature importance -- if we figure out those error bars --, what kind of examples get routed to kge vs. lm, or to one lm vs. another lm... etc.}
\begin{itemize}
    \item Ensembling best LM with best baselines improves results, with varying improvement across datasets
    \item Best ensemble is almost always combination of a KGE model and an LM, rather than two KGE models
    \item (Possibly) Also include results ensembling multiple LMs, or multiple LMs and a KGE model? \tom{if this helps results, then sure! we haven't seen others doing this}
\end{itemize}

\subsection{Inductive knowledge graph completion}
\tom{for the case with only one missing entity, do you use the actual KGE embedding for the entity that is not missing? not random - right?}

\tom{discuss why we don't compare to other inductive kgc approaches (that are based on paths etc.)}
\begin{itemize}
    \item One advantage of LM-based KG completion is the ability to infer compositional entity representations from text alone, can apply to unseen entities at test time
    \item We also constructed inductive splits of same three datasets to test this property (every validation/test example has either one or both entities unseen in the training set)
\end{itemize}

\subsubsection{Results}

\begin{itemize}
    \item Language models perform worse on inductive split than they do in the transductive setting, but still do better than random KG embeddings (as expected)
    \item (Possibly) Using nearest-neighbor entity representations from PubMedBERT to fill in missing entities improves performance of KGE models (not sure about this, still need to run experiments!) \tom{if we do this, should also try string matching and see if p-bert does better; can also compare p-bert pretrained vs. kg-p-bert after fine-tuning}
    \item (Possibly) Maybe show examples of unseen entities/triples where language models do well?
\end{itemize}
